Autoencoders as Tools for Program Synthesis

Recently there have been many advances in research on language modeling of source code. Applications range from code suggestion and completion to code summarization. However, complete program synthesis of industry-grade programming languages remains an open problem. In this work, we introduce and experimentally validate a variational autoencoder model for program synthesis of industry-grade programming languages. This model makes use of the inherent tree structure of code and can be used in conjunction with gradient free optimization techniques like evolutionary methods to generate programs that maximize a given fitness function, for instance, passing a set of test cases. A demonstration is avaliable at https://tree2tree.app

==> Seq2Seq.tex <==
In this section, we present a baseline autoencoder model for program synthesis. The baseline model is meant to serve as a reference model to compare its performance against the proposed autoencoder model that will be presented in the next section. The baseline model is inspired by autoencoders used for text generation in natural language. By taking inspiration from natural language models, we can also evaluate how well these models generalize to source code synthesis. 

\subsection{Architecture}

The baseline model considered takes inspiration from NLP autoencoder models. Typically, NLP methods consider texts/inputs as linear sequences of tokens. Our baseline model will follow this approach and consider source code as a sequence. The model will take a sequence as input and output a sequence. Therefore, we refer to the baseline model as the sequence to sequence model or Seq2Seq in short. In this work, we will focus on Variational Autoencoders (VAE) to allow for the generation of new programs, as discussed in \cref{sec:VAE}

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/seq2seq.png}
    \caption{The architecture of the Seq2Seq model}
    \label{fig:seq2seq}
\end{figure*}



The model architecture is inspired from \cite{bowman2015generating}. In this architecture, both the encoder and decoder networks contain single-layer recurrent neural networks. A Gaussian prior is used for the regularization of the latent space. The decoder is an RNN language model that is conditioned on the latent code that the encoder outputs. More specifically, the encoder takes the hidden state of its RNN after operating on a sequence and outputs a mean and variance. After obtaining a mean and variance from the encoder, we sample a latent code $z$ representing the input using the reparameterization trick \cite{kingma2013auto}. The decoder uses $z$ and transforms it to a state, with the help of a linear layer, where it can be used as initial the hidden state for its RNN. This architecture is depicted in \cref{fig:seq2seq}. In the model, tokens are represented using a learned dictionary of embedding vectors. These embedding vectors can either be learned from scratch or pre-trained and then fine-tuned. 

\subsection{Optimization}
The model aims to learn a latent space that represents source code. We can quantify how well the model learns a latent space using a variational lower bound objective \cref{eq:ELBO}. This bound can be expressed as two separate terms: the likelihood of the data under the posterior (which we refer to as the reconstruction loss) and KL divergence. Simply put, the reconstruction loss is a measure of how well the model reconstructs the input, while the KL divergence is a measure of how similar the posterior is compared to the prior. A common issue of variational autoencoders, where the decoder is parameterized with an auto-regressive model, is KL vanishing \cite{bowman2015generating}. The KL divergence term will go to zero when this happens, and the model will behave as an RNN language model. We employ two techniques to mitigate this issue. 

\subsubsection{Cyclic KL annealing}\label{seq2seq:cyclic_kl_annealing}
We employ cyclical KL cost annealing \cite{fu2019cyclical} to mitigate the KL vanishing issue.
This technique weighs the KL divergence term of the loss function, increasing the weight from 0 to 1 at a fast pace, staying at 1 for some iterations, and then returning to 0 in several cycles. The cyclical schedule can progressively improve the performance by resetting the KL term to 0 to leverage good latent codes learned in previous cycles as warm re-starts. 

\subsubsection{Word dropout}
As in \cite{bowman2015generating}, we use a technique called word (or token) dropout. The cyclic KL annealing weakens the penalty term on the output of the encoder whereas word dropout weakens the decoder. The decoder learns how to predict a next token conditioned on the true previous token using teacher forcing. To weaken the decoder, some of the information of the conditioning can be removed during learning. This can be achieved by randomly replacing a fraction of the previous true tokens with an unknown token. This is a technique to force the model to rely on the latent variable $z$ for learning how to reconstruct the input. The fraction of true tokens replaced by unknown tokens is a hyperparameter between 0 and 1. When this hyperparameter is set to 1, the decoder sees no input.  

\subsubsection{Loss function}
The last part of the model that has yet to be defined is the loss function. The KL divergence part of the loss function can be computed in closed form given our Gaussian prior (\Cref{eq:KL_div}). We use the output of the encoder, the mean and variance, to compute the KL divergence. We use cross-entropy loss (negative log-likelihood) between the softmax probabilities of the predicted sequence of the encoder and the target sequence (reconstruction) to estimate the reconstruction loss. Our dataset contains almost 300.000 unique tokens, and the distribution of these tokens is highly imbalanced. For example, the token "\{" occurs much more often than an arbitrary user-defined variable name. Therefore, to allow softmax to be computed efficiently, we use adaptive softmax \cite{grave2017efficient}. The reconstruction loss and KL divergence term are then summed, and this total cost function is optimized during training.

\subsection{Data Pre-processing}
The data set containing complete C++ programs must be pre-processed to sequences of tokens to feed the model. This pre-processing step must be reversible up to a particular state. More specifically, we need to create syntactically valid and compilable programs back from the sequences of tokens. Furthermore, the reconstructed programs should not function any differently compared to their original counterparts.



We want to model to learn how to generate valid code. Therefore, we remove certain components from programs that are not we do not consider as source code. These components are comments, imports/includes, and macros. Comments can safely be removed without changing the functionality of a program. Imports can be extracted, saved, and re-added later, if necessary. Additionally, we expand any defined macros in the source code. We expand the macros and remove comments by running CLANG C++ compiler with the `-E' option, which stops the compiler after the prepossessing stage.



==> data.tex <==
There are a few requirements that a data set should adhere to for making training an autoencoder successful or even possible. One of the key goals of this research is that we want to create an autoencoder model that can generate syntactically correct and compile-able code. Therefore, it is of importance that the data the model is trained on also exhibits these properties. Any source code that the model is trained on should be a functional piece of code that can be compiled and run. Furthermore, we want to experiment with creating an autoencoder model to generate code in industry-grade programming languages; therefore, the data set has to contain only source code of an industry-grade programming language. Next, the autoencoder should learn how to model the syntax and structure of a programming language. To make this most effective, similar to NLP methods, we focus on a single language. Lastly, any source code the model is trained on should be standalone source code. Standalone in the sense that the source code should not be part of some larger code base but contains all necessary components, excluding any imports key to the language.



\noindent To summarize, the data set should adhere to the following requirements:

\begin{itemize}
    \item The data should contain only syntactically correct and compile-able source code
    \item The data should contain only source code of a single industry-grade programming language
    \item The data should contain only standalone source code (excluding any imports to libraries built into the language)
\end{itemize}



Code competition websites collect data that follow all the requirements mentioned above. These platforms collect and test source code that is meant to solve a predefined problem. Contests may be held on these platforms, possibly containing multiple problems that should be solved. Contenders may then use any programming language that the platform supports to solve the problem and upload their solution. The platform will then check the solution against some tests defined with the problem and give the user a score or indication of whether the solution solves the problem. 

\begin{table}[ht!]
\centering
% A table with adjusted row and column spacings
% \setlength sets the horizontal (column) spacing
% \arraystretch sets the vertical (row) spacing
\begingroup
\setlength{\tabcolsep}{8pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.6} % Default value: 1
\begin{tabular}{c|ccccc}
  & \textbf{Total} & \textbf{Mean \#} & \textbf{Median \#} & \textbf{Min \#} & \textbf{Max \#} \\ \hline
\textbf{Contests} & 148 & 13,277 & 13,383 & 36 & 51,460 \\
\textbf{Problems} & 904 & 2174 & 898 & 1 & 19,790 \\
\end{tabular}
\caption[Data set statistics]{Data set statistics in terms of number of contests, problems and statistics on number of programs within contests and problems.}
\label{tab:statistics_contests_problems}
\endgroup
\end{table}



As mentioned before, we require the programs in our data set to be standalone source code, as do the code competition platforms. Therefore, the programs minimally contain a main function, as the C++ language requires this. For most programs in the data, all of the functionality is included in this main function. Nevertheless, some programs use other C++ elements such as helper functions, classes, or enumerations. 



The code competition platforms use the standard input and standard output of programming languages to communicate with the participant's programs. Combinations of input and output are defined as various tests to evaluate whether the programs conform to the specifications. Therefore, the standard input and output streams of C++, $cin$ and $cout$, respectively, are elements that are always present in each program of our data set. 



Additionally, answers to the code competition problems are limited in terms of memory usage and computation time. For this reason, the programs often contain optimizations. Examples of optimizations for computation time are disabling the synchronization between the C and C++ standard streams and decoupling the input and output stream. Furthermore, examples of optimizations in terms of memory are the usage of bit-wise operations and smaller data types. 



To conclude, the programs in the data set are generally structured to contain a main function, standard input and output stream elements, computation and memory optimizations, and possibly some other elements such as helper functions/classes. Due to this general structure, the programs tend to overlap in their content, in contrast to, for example, natural language sentences. 
